Dimension-Free Average Treatment Effect Inference with Deep Neural Networks

This paper investigates the estimation and inference of the average treatment effect (ATE) using deep neural networks (DNNs) in the potential outcomes framework. Under some regularity conditions, the observed response can be formulated as the response of a mean regression problem with both the confounding variables and the treatment indicator as the independent variables. Using such formulation, we investigate two methods for ATE estimation and inference based on the estimated mean regression function via DNN regression using a specific network architecture. We show that both DNN estimates of ATE are consistent with dimension-free consistency rates under some assumptions on the underlying true mean regression model. Our model assumptions accommodate the potentially complicated dependence structure of the observed response on the covariates, including latent factors and nonlinear interactions between the treatment indicator and confounding variables. We also establish the asymptotic normality of our estimators based on the idea of sample splitting, ensuring precise inference and uncertainty quantification. Simulation studies and real data application justify our theoretical findings and support our DNN estimation and inference methods.

==> real_data_figs_tables/ATE_DNN_real_data_pension_results_table.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{cccccc}
\toprule
Inference Proportion & Training Epochs & Estimate Type & Activation & Median & Robust SD\\
\midrule
 &  &  & ReLU & 7328 & 2008\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6300 & 2261\\
\cmidrule{3-6}
 &  &  & ReLU & 8683 & 3528\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8114 & 3052\\
\cmidrule{2-6}
 &  &  & ReLU & 7711 & 1664\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6462 & 2212\\
\cmidrule{3-6}
 &  &  & ReLU & 8200 & 3410\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7495 & 3057\\
\cmidrule{2-6}
 &  &  & ReLU & 7780 & 2362\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6911 & 2442\\
\cmidrule{3-6}
 &  &  & ReLU & 7440 & 4488\\

\multirow{-12}{*}{\centering\arraybackslash 0.2} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8025 & 3384\\
\cmidrule{1-6}
 &  &  & ReLU & 7624 & 2154\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 5960 & 2152\\
\cmidrule{3-6}
 &  &  & ReLU & 8159 & 2349\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8281 & 2084\\
\cmidrule{2-6}
 &  &  & ReLU & 7761 & 2252\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6650 & 2115\\
\cmidrule{3-6}
 &  &  & ReLU & 7987 & 2547\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8118 & 2252\\
\cmidrule{2-6}
 &  &  & ReLU & 7400 & 2669\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6659 & 2036\\
\cmidrule{3-6}
 &  &  & ReLU & 8127 & 3460\\

\multirow{-12}{*}{\centering\arraybackslash 0.3} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7723 & 2289\\
\cmidrule{1-6}
 &  &  & ReLU & 7546 & 2428\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6526 & 2443\\
\cmidrule{3-6}
 &  &  & ReLU & 8220 & 2301\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8013 & 1689\\
\cmidrule{2-6}
 &  &  & ReLU & 8064 & 2518\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6722 & 1942\\
\cmidrule{3-6}
 &  &  & ReLU & 7970 & 2257\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7840 & 1967\\
\cmidrule{2-6}
 &  &  & ReLU & 8201 & 2871\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6764 & 2429\\
\cmidrule{3-6}
 &  &  & ReLU & 7497 & 3310\\

\multirow{-12}{*}{\centering\arraybackslash 0.4} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7614 & 2035\\
\cmidrule{1-6}
 &  &  & ReLU & 7472 & 1831\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 5819 & 2208\\
\cmidrule{3-6}
 &  &  & ReLU & 8292 & 1960\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8184 & 1462\\
\cmidrule{2-6}
 &  &  & ReLU & 7676 & 2400\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6571 & 2456\\
\cmidrule{3-6}
 &  &  & ReLU & 7935 & 2332\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7959 & 1505\\
\cmidrule{2-6}
 &  &  & ReLU & 7473 & 3743\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 6549 & 2438\\
\cmidrule{3-6}
 &  &  & ReLU & 7934 & 4051\\

\multirow{-12}{*}{\centering\arraybackslash 0.5} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7603 & 1872\\
\bottomrule
\end{tabular}}
\end{table}


==> real_data_figs_tables/ATE_DNN_real_data_pension_results_table_num_epochs_100.tex <==

\begin{tabular}[t]{ccccc}
\toprule
Training Proportion & Estimate Type & Activation & Median & Robust SD\\
\midrule
 &  & ReLU & 1801 & 1224\\
\cmidrule{3-5}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 1716 & 803\\
\cmidrule{2-5}
 &  & ReLU & 11305 & 4457\\
\cmidrule{3-5}
\multirow{-4}{*}{\centering\arraybackslash 0.2} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 7286 & 7653\\
\cmidrule{1-5}
 &  & ReLU & 3734 & 1407\\
\cmidrule{3-5}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 3215 & 1631\\
\cmidrule{2-5}
 &  & ReLU & 9369 & 4072\\
\cmidrule{3-5}
\multirow{-4}{*}{\centering\arraybackslash 0.3} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 6676 & 6216\\
\cmidrule{1-5}
 &  & ReLU & 5452 & 1800\\
\cmidrule{3-5}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 4581 & 1494\\
\cmidrule{2-5}
 &  & ReLU & 9187 & 4142\\
\cmidrule{3-5}
\multirow{-4}{*}{\centering\arraybackslash 0.4} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 8163 & 5320\\
\bottomrule
\end{tabular}


==> sim_1_figs_tables/ATE_DNN_sim_1_results_table.tex <==

\begin{tabular}[t]{ccccccc}
\toprule
N & Training Epochs & Activation & Mean & Median & SD & MSE\\
\midrule
 &  & ReLU & 0.9808 & 0.9791 & 0.09563 & 0.00947\\

 & \multirow{-2}{*}{\centering\arraybackslash 100} & Sigmoid & 0.9239 & 0.9236 & 0.09009 & 0.01386\\
\cmidrule{2-7}
 &  & ReLU & 0.9847 & 0.9844 & 0.11223 & 0.01277\\

 & \multirow{-2}{*}{\centering\arraybackslash 200} & Sigmoid & 0.9555 & 0.9566 & 0.06773 & 0.00654\\
\cmidrule{2-7}
 &  & ReLU & 0.9670 & 0.9656 & 0.10374 & 0.01180\\

 & \multirow{-2}{*}{\centering\arraybackslash 400} & Sigmoid & 0.9764 & 0.9726 & 0.06355 & 0.00457\\
\cmidrule{2-7}
 &  & ReLU & 0.9567 & 0.9592 & 0.09532 & 0.01091\\

\multirow{-8}{*}{\centering\arraybackslash 1000} & \multirow{-2}{*}{\centering\arraybackslash 800} & Sigmoid & 1.0196 & 1.0175 & 0.07522 & 0.00601\\
\cmidrule{1-7}
 &  & ReLU & 0.9807 & 0.9815 & 0.07616 & 0.00614\\

 & \multirow{-2}{*}{\centering\arraybackslash 100} & Sigmoid & 0.9479 & 0.9503 & 0.04731 & 0.00494\\
\cmidrule{2-7}
 &  & ReLU & 0.9823 & 0.9872 & 0.07756 & 0.00630\\

 & \multirow{-2}{*}{\centering\arraybackslash 200} & Sigmoid & 0.9672 & 0.9675 & 0.04974 & 0.00354\\
\cmidrule{2-7}
 &  & ReLU & 0.9692 & 0.9711 & 0.07743 & 0.00692\\

 & \multirow{-2}{*}{\centering\arraybackslash 400} & Sigmoid & 0.9917 & 0.9913 & 0.05239 & 0.00280\\
\cmidrule{2-7}
 &  & ReLU & 0.9760 & 0.9703 & 0.07188 & 0.00572\\

\multirow{-8}{*}{\centering\arraybackslash 2000} & \multirow{-2}{*}{\centering\arraybackslash 800} & Sigmoid & 0.9927 & 0.9864 & 0.05797 & 0.00340\\
\cmidrule{1-7}
 &  & ReLU & 0.9867 & 0.9864 & 0.06919 & 0.00494\\

 & \multirow{-2}{*}{\centering\arraybackslash 100} & Sigmoid & 0.9612 & 0.9597 & 0.04027 & 0.00312\\
\cmidrule{2-7}
 &  & ReLU & 0.9877 & 0.9851 & 0.07042 & 0.00508\\

 & \multirow{-2}{*}{\centering\arraybackslash 200} & Sigmoid & 0.9771 & 0.9760 & 0.03771 & 0.00194\\
\cmidrule{2-7}
 &  & ReLU & 0.9711 & 0.9687 & 0.07216 & 0.00602\\

 & \multirow{-2}{*}{\centering\arraybackslash 400} & Sigmoid & 0.9958 & 0.9974 & 0.04351 & 0.00190\\
\cmidrule{2-7}
 &  & ReLU & 0.9837 & 0.9776 & 0.07215 & 0.00544\\

\multirow{-8}{*}{\centering\arraybackslash 3000} & \multirow{-2}{*}{\centering\arraybackslash 800} & Sigmoid & 0.9911 & 0.9899 & 0.04983 & 0.00255\\
\cmidrule{1-7}
 &  & ReLU & 0.9754 & 0.9756 & 0.05937 & 0.00411\\

 & \multirow{-2}{*}{\centering\arraybackslash 100} & Sigmoid & 0.9627 & 0.9601 & 0.03353 & 0.00251\\
\cmidrule{2-7}
 &  & ReLU & 0.9837 & 0.9764 & 0.06929 & 0.00504\\

 & \multirow{-2}{*}{\centering\arraybackslash 200} & Sigmoid & 0.9779 & 0.9779 & 0.03706 & 0.00186\\
\cmidrule{2-7}
 &  & ReLU & 0.9903 & 0.9834 & 0.06273 & 0.00401\\

 & \multirow{-2}{*}{\centering\arraybackslash 400} & Sigmoid & 0.9930 & 0.9932 & 0.03933 & 0.00159\\
\cmidrule{2-7}
 &  & ReLU & 0.9769 & 0.9740 & 0.06647 & 0.00493\\

\multirow{-8}{*}{\centering\arraybackslash 4000} & \multirow{-2}{*}{\centering\arraybackslash 800} & Sigmoid & 0.9881 & 0.9926 & 0.04098 & 0.00181\\
\cmidrule{1-7}
 &  & ReLU & 0.9883 & 0.9911 & 0.06214 & 0.00398\\

 & \multirow{-2}{*}{\centering\arraybackslash 100} & Sigmoid & 0.9636 & 0.9614 & 0.03735 & 0.00271\\
\cmidrule{2-7}
 &  & ReLU & 0.9806 & 0.9850 & 0.06339 & 0.00437\\

 & \multirow{-2}{*}{\centering\arraybackslash 200} & Sigmoid & 0.9732 & 0.9725 & 0.03404 & 0.00187\\
\cmidrule{2-7}
 &  & ReLU & 0.9741 & 0.9773 & 0.06648 & 0.00507\\

 & \multirow{-2}{*}{\centering\arraybackslash 400} & Sigmoid & 0.9971 & 0.9986 & 0.03195 & 0.00102\\
\cmidrule{2-7}
 &  & ReLU & 0.9821 & 0.9866 & 0.06029 & 0.00394\\

\multirow{-8}{*}{\centering\arraybackslash 5000} & \multirow{-2}{*}{\centering\arraybackslash 800} & Sigmoid & 0.9941 & 0.9931 & 0.04124 & 0.00173\\
\bottomrule
\end{tabular}


==> sim_2_figs_tables/ATE_DNN_sim_2_results_table.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{cccccccc}
\toprule
N & Training Epochs & Estimate Type & Activation & Mean & Median & SD & MSE\\
\midrule
 &  &  & ReLU & 0.9763 & 0.9767 & 0.09150 & 0.00889\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9172 & 0.9251 & 0.09622 & 0.01607\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9703 & 0.9659 & 0.16154 & 0.02684\\

 & \multirow{-4}{*}{\centering\arraybackslash 100} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9808 & 0.9788 & 0.08293 & 0.00721\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9735 & 0.9764 & 0.09660 & 0.00999\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9553 & 0.9565 & 0.07190 & 0.00714\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9602 & 0.9495 & 0.17878 & 0.03339\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9654 & 0.9649 & 0.08281 & 0.00802\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9764 & 0.9798 & 0.09930 & 0.01037\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9833 & 0.9834 & 0.07282 & 0.00556\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9809 & 0.9732 & 0.18509 & 0.03445\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9626 & 0.9633 & 0.08055 & 0.00785\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9665 & 0.9751 & 0.10528 & 0.01215\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 1.0177 & 1.0193 & 0.07743 & 0.00628\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9757 & 0.9716 & 0.19882 & 0.03992\\

\multirow{-16}{*}{\centering\arraybackslash 1000} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9620 & 0.9631 & 0.08996 & 0.00949\\
\cmidrule{1-8}
 &  &  & ReLU & 0.9707 & 0.9692 & 0.07016 & 0.00575\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9467 & 0.9516 & 0.04716 & 0.00505\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9891 & 0.9851 & 0.17272 & 0.02980\\

 & \multirow{-4}{*}{\centering\arraybackslash 100} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9742 & 0.9669 & 0.07878 & 0.00684\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9767 & 0.9787 & 0.07471 & 0.00610\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9626 & 0.9655 & 0.04696 & 0.00359\\
\cmidrule{3-8}
 &  &  & ReLU & 1.0010 & 0.9830 & 0.17861 & 0.03174\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9718 & 0.9620 & 0.08075 & 0.00728\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9666 & 0.9646 & 0.08197 & 0.00780\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9869 & 0.9904 & 0.04714 & 0.00238\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9948 & 0.9835 & 0.18331 & 0.03346\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9678 & 0.9692 & 0.08182 & 0.00770\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9750 & 0.9771 & 0.07266 & 0.00588\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9840 & 0.9843 & 0.05472 & 0.00324\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9792 & 0.9743 & 0.17514 & 0.03095\\

\multirow{-16}{*}{\centering\arraybackslash 2000} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9751 & 0.9715 & 0.08919 & 0.00854\\
\cmidrule{1-8}
 &  &  & ReLU & 0.9845 & 0.9852 & 0.06145 & 0.00400\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9626 & 0.9615 & 0.03774 & 0.00282\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9880 & 0.9795 & 0.14298 & 0.02049\\

 & \multirow{-4}{*}{\centering\arraybackslash 100} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9678 & 0.9657 & 0.07579 & 0.00675\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9862 & 0.9814 & 0.07825 & 0.00628\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9749 & 0.9722 & 0.03776 & 0.00205\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9711 & 0.9655 & 0.13425 & 0.01876\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9688 & 0.9657 & 0.07743 & 0.00694\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9770 & 0.9660 & 0.06987 & 0.00538\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9959 & 0.9971 & 0.04165 & 0.00174\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9689 & 0.9614 & 0.17931 & 0.03296\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9660 & 0.9647 & 0.08015 & 0.00755\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9785 & 0.9808 & 0.07092 & 0.00547\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9896 & 0.9882 & 0.04791 & 0.00239\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9772 & 0.9881 & 0.13725 & 0.01926\\

\multirow{-16}{*}{\centering\arraybackslash 3000} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9754 & 0.9749 & 0.08674 & 0.00809\\
\cmidrule{1-8}
 &  &  & ReLU & 0.9813 & 0.9812 & 0.06223 & 0.00420\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9597 & 0.9590 & 0.03335 & 0.00273\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9884 & 0.9975 & 0.13479 & 0.01821\\

 & \multirow{-4}{*}{\centering\arraybackslash 100} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9695 & 0.9662 & 0.07448 & 0.00645\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9766 & 0.9699 & 0.06312 & 0.00451\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9695 & 0.9694 & 0.03313 & 0.00202\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9826 & 0.9743 & 0.13325 & 0.01797\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9699 & 0.9596 & 0.07169 & 0.00602\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9802 & 0.9814 & 0.06417 & 0.00449\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9888 & 0.9895 & 0.03778 & 0.00155\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9723 & 0.9590 & 0.15317 & 0.02411\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9696 & 0.9696 & 0.07448 & 0.00645\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9773 & 0.9819 & 0.06328 & 0.00450\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9837 & 0.9852 & 0.04295 & 0.00210\\
\cmidrule{3-8}
 &  &  & ReLU & 1.0051 & 0.9869 & 0.16570 & 0.02735\\

\multirow{-16}{*}{\centering\arraybackslash 4000} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9785 & 0.9753 & 0.08152 & 0.00707\\
\cmidrule{1-8}
 &  &  & ReLU & 0.9892 & 0.9930 & 0.05888 & 0.00357\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9639 & 0.9640 & 0.02923 & 0.00215\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9941 & 0.9972 & 0.11426 & 0.01302\\

 & \multirow{-4}{*}{\centering\arraybackslash 100} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9759 & 0.9810 & 0.06615 & 0.00494\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9854 & 0.9844 & 0.06355 & 0.00423\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9729 & 0.9737 & 0.03164 & 0.00173\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9893 & 0.9891 & 0.12253 & 0.01505\\

 & \multirow{-4}{*}{\centering\arraybackslash 200} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9752 & 0.9776 & 0.06742 & 0.00514\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9864 & 0.9919 & 0.06906 & 0.00493\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9931 & 0.9944 & 0.03044 & 0.00097\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9928 & 0.9943 & 0.12544 & 0.01571\\

 & \multirow{-4}{*}{\centering\arraybackslash 400} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9780 & 0.9852 & 0.06821 & 0.00511\\
\cmidrule{2-8}
 &  &  & ReLU & 0.9874 & 0.9886 & 0.06703 & 0.00463\\

 &  & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9941 & 0.9953 & 0.03458 & 0.00122\\
\cmidrule{3-8}
 &  &  & ReLU & 0.9843 & 0.9710 & 0.13930 & 0.01955\\

\multirow{-16}{*}{\centering\arraybackslash 5000} & \multirow{-4}{*}{\centering\arraybackslash 800} & \multirow{-2}{*}{\centering\arraybackslash Doubly Robust Estimate} & Sigmoid & 0.9857 & 0.9902 & 0.07306 & 0.00552\\
\bottomrule
\end{tabular}}
\end{table}


==> sim_2_figs_tables/test.tex <==

\begin{tabular}[t]{ccccccc}
\toprule
N & Estimate Type & Activation & Mean & Median & SE & MSE\\
\midrule
 &  & ReLU & 0.9705 & 0.9674 & 0.00102 & 0.01129\\
\cmidrule{3-7}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 1.0142 & 1.0262 & 0.00078 & 0.00632\\
\cmidrule{2-7}
 &  & ReLU & 1.1745 & 1.4073 & 0.02710 & 7.33585\\
\cmidrule{3-7}
\multirow{-4}{*}{\centering\arraybackslash 1000} & \multirow{-2}{*}{\centering\arraybackslash IPW Estimate} & Sigmoid & 0.9674 & 0.9717 & 0.00083 & 0.00800\\
\cmidrule{1-7}
 &  & ReLU & 0.9693 & 0.9766 & 0.00080 & 0.00730\\
\cmidrule{3-7}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9846 & 0.9849 & 0.00057 & 0.00345\\
\cmidrule{2-7}
 &  & ReLU & 1.1438 & 0.9822 & 0.02610 & 6.79670\\
\cmidrule{3-7}
\multirow{-4}{*}{\centering\arraybackslash 2000} & \multirow{-2}{*}{\centering\arraybackslash IPW Estimate} & Sigmoid & 0.9839 & 0.9807 & 0.00085 & 0.00750\\
\cmidrule{1-7}
 &  & ReLU & 0.9800 & 0.9822 & 0.00069 & 0.00511\\
\cmidrule{3-7}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9912 & 0.9904 & 0.00047 & 0.00231\\
\cmidrule{2-7}
 &  & ReLU & 1.5632 & 1.6086 & 0.02553 & 6.80234\\
\cmidrule{3-7}
\multirow{-4}{*}{\centering\arraybackslash 3000} & \multirow{-2}{*}{\centering\arraybackslash IPW Estimate} & Sigmoid & 0.9826 & 0.9831 & 0.00086 & 0.00764\\
\cmidrule{1-7}
 &  & ReLU & 0.9888 & 0.9881 & 0.00071 & 0.00520\\
\cmidrule{3-7}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9861 & 0.9868 & 0.00039 & 0.00174\\
\cmidrule{2-7}
 &  & ReLU & 0.8305 & 0.9437 & 0.02321 & 5.38724\\
\cmidrule{3-7}
\multirow{-4}{*}{\centering\arraybackslash 4000} & \multirow{-2}{*}{\centering\arraybackslash IPW Estimate} & Sigmoid & 0.9882 & 0.9911 & 0.00080 & 0.00652\\
\cmidrule{1-7}
 &  & ReLU & 0.9859 & 0.9901 & 0.00062 & 0.00406\\
\cmidrule{3-7}
 & \multirow{-2}{*}{\centering\arraybackslash Difference of Means Estimate} & Sigmoid & 0.9921 & 0.9955 & 0.00034 & 0.00122\\
\cmidrule{2-7}
 &  & ReLU & 1.1944 & 1.2893 & 0.01792 & 3.23172\\
\cmidrule{3-7}
\multirow{-4}{*}{\centering\arraybackslash 5000} & \multirow{-2}{*}{\centering\arraybackslash IPW Estimate} & Sigmoid & 0.9952 & 0.9920 & 0.00074 & 0.00541\\
\bottomrule
\end{tabular}

